Randomized contractions meet lean decompositions

We show an algorithm that, given an $n$-vertex graph $G$ and a parameter $k$, in time $2^{O(k \log k)} n^{O(1)}$ finds a tree decomposition of $G$ with the following properties: * every adhesion of the tree decomposition is of size at most $k$, and * every bag of the tree decomposition is $(i,i)$-unbreakable in $G$ for every $1 \leq i \leq k$. Here, a set $X \subseteq V(G)$ is $(a,b)$-unbreakable in $G$ if for every separation $(A,B)$ of order at most $b$ in $G$, we have $|A \cap X| \leq a$ or $|B \cap X| \leq a$. The resulting tree decomposition has arguably best possible adhesion size boundsand unbreakability guarantees. Furthermore, the parametric factor in the running time bound is significantly smaller than in previous similar constructions. These improvements allow us to present parameterized algorithms for Minimum Bisection, Steiner Cut, and Steiner Multicut with improved parameteric factor in the running time bound. The main technical insight is to adapt the notion of lean decompositions of Thomas and the subsequent construction algorithm of Bellenbaum and Diestel to the parameterized setting.

==> algo-multicut.tex <==
We now apply the framework to the \textsc{Steiner Multicut} problem.
In this problem we are given an undirected graph $G$, $t$ sets of terminals $T_1,T_2,\ldots,T_t$, each of size at most $p$,
   and an integer $k$. The goal is to delete at most $k$ edges from $G$ such that every terminal set $T_i$ is separated:
   for every $1 \leq i \leq t$, there does not exist a single connected component of the resulting graph that contains the
   entire set $T_i$. 
Note that for $p=2$, the problem becomes the classic \textsc{Edge Multicut} problem.

Bringmann et al~\cite{BringmannHML16} showed an FPT algorithm for \textsc{Steiner Multicut} when parameterized by $k+t$.
We use our decomposition theorem to improve the exponential part of the running time of this algorithm.
\begin{theorem}\label{thm:multicut}
\textsc{Steiner Multicut} can be solved in time $2^{\Oh((t + k) \log (k + t))} |V(G)|^{\Oh(1)}$.
\end{theorem}

\begin{proof}
Let $(G,(T_i)_{i=1}^t,k)$ be an input to \textsc{Steiner Multicut} and let $n = |V(G)|$.
Let $p = \max_{i=1}^t |T_i|$. 

First, we observe that it is sufficient to solve \textsc{Steiner Multicut} with the additional assumption that $G$ is connected.
Indeed, in the general case we can proceed as follows. First, we discard all sets $T_i$ that intersect more than one connected component of $G$. Second, for every connected component $G'$ of $G$ and every $0 \leq k' \leq k$, we solve \textsc{Steiner Multicut}
on graph $G$, terminal sets $\{T_i~|~T_i \subseteq V(G')\}$, and budget $k'$.
Finally, the results of these computations allow us to solve the input instance by a straightforward knapsack-type
dynamic programming algorithm.
Thus, henceforth we assume that $G$ is connected.

Assume we are given a graph $H$ and a function $f : V(H) \to [k+1]$.
The \emph{cost} of $f$ on $H$
is defined as the number of edges $uv \in E(H)$ with $f(u) \neq f(v)$
and denoted as $\fcost_H(f)$.
We say that $f$ is \emph{non-monochromatic} on a set $W \subseteq V(G)$
if there exists two elements $t_1,t_2 \in W$ with $f(t_1) \neq f(t_2)$.
Since $G$ is connected, removal of at most $k$ edges can lead to at most $k+1$ connected components.
Therefore, one can rephrase the \textsc{Steiner Multicut} problem on $(G,(T_i)_{i=1}^t,k)$ as follows:
does there exist a function $f : V(G) \to [k+1]$ of cost at most $k$ that is
non-monochromatic on each set $T_i$.

We further reformulate the question 
For every $i \in [t]$ we pick a representative $s_i \in T_i$ and let $S = \{s_i~|~i \in [t]\}$.
We iterate over all functions $f_S : S \to [k+1]$; there are $(k+1)^{|S|} \leq (k+1)^t$ of them.
For a fixed function $f_S$, we ask for a function $f: V(G) \to [k+1]$ of cost at most $k$ that extends $f_S$
and such that for every $i \in [t]$ there exists $w_i \in T_i$ with $f(w_i) \neq f(s_i)$.
For fixed $f_S$, we call such a function $f$ \emph{a solution}.

Clearly, the input instance $(G,(T_i)_{i=1}^t,k)$ is a yes-instance if and only if there exists $f_S : S \to [k+1]$
for which there exists a solution.
Henceforth we fix vertices $s_i$ and a function $f_S : S \to [k+1]$ and look for a solution.

We invoke the algorithm of Theorem~\ref{thm:decomp} to $G$ and $k$,
obtaining a rooted compact
tree decomposition $(T,\beta)$ of $G$ whose every bag is $(k,k)$-edge-unbreakable
and every adhesion is of size at most $k$. The running time of this step 
is $2^{\Oh(k \log k)} n^{\Oh(1)}$.

We perform a bottom-up dynamic programming algorithm on $(T,\beta)$. 
For every node $t \in V(T)$, every subset $I \subseteq [t]$, and every
function $f^\adh: \adh(t) \to [k+1]$ that agrees with $f_S$ on $\adh(t) \cap S$, we compute a value $M[t, I, f^\adh] \in \{0, 1, 2, \ldots, k, +\infty\}$
with the following properties.

\begin{enumerate}[label={(\alph*)}]
\item If $M[t,I, f^\adh] \neq +\infty$, then there exists a function $f : V(G_t) \to [k+1]$ such that:\label{i:mc:cmpl}
\begin{itemize}
\item $f|_{\adh(t)} = f^\adh$ and $f|_{S \cap V(G_t)} = f_S|_{S \cap V(G_t)}$
\item for every $i \in I$ there exists $w_i \in V(G_t) \cap T_i$ with $f(w_i) \neq f_S(s_i)$;
\item the cost of $f$ in $G_t$ is at most $M[t,I,f^\adh]$.
\end{itemize}
\item For every function $f : V(G) \to [k+1]$ that satisfies:\label{i:mc:sound}
\begin{itemize}
\item $f|_{\adh(t)} = f^\adh$ and $f|_S = f_S$,
\item for every $i \in [t]$ there exists $w_i \in T_i$ with $f(w_i) \neq f_S(s_i)$, and, 
  furthermore, if $i \in I$ there exists $w_i \in T_i \cap V(G_t)$ with $f(w_i) \neq f_S(s_i)$,
\item the cost of $f$ in $G$ is at most $k$,
\end{itemize}
the cost of $f|_{V(G_t)}$ in $G_t$ is at least $M[t,I,f^\adh]$.
\end{enumerate}

We first observe that the table $M[\cdot]$ is sufficient for our purposes.
\begin{claim}\label{cl:mc:M}
There exists a solution if and only if
$M[r,[t],\emptyset] \neq +\infty$ for the root $r$ of $T$.
\end{claim}
\begin{proof}
In one direction, if $f$ is a solution, then note that
$f$ satisfies all conditions of Point~\ref{i:mc:sound} for the cell
$M[r,[t],\emptyset]$. Hence, by Point~\ref{i:mc:sound}, $M[r,[t],\emptyset] < +\infty$.

In the other direction, let $M[r,[t],\emptyset] < +\infty$ and 
let $f$ be the function whose existence is asserted by Point~\ref{i:mc:cmpl}.
Then for every $i \in [t]$ there exists $w_i \in T_i$ with $f(w_i) \neq f_S(s_i)$ and its cost in $G_r = G$ is at most $k$.
Consequently, $f$ is a solution.
\cqed\end{proof}

Thus, to prove Theorem~\ref{thm:multicut}, it suffices to show how to compute in time
$2^{\Oh((t + k) \log (k + t))} n^{\Oh(1)}$ entries $M[t,\cdot,\cdot]$ for a fixed node $t \in V(T)$, given
entries $M[s,\cdot,\cdot]$ for all children $s$ of $t$ in $T$. Since $|\adh(t)| \leq k$,
it suffices to focus on a computation of a single cell $M[t,I,f^\adh]$.
Let $Z$ be the set of children of $t$ in $T$.

In a single step of a dynamic programming algorith, we would like to focus on finding
a function $f^\beta : \beta(t) \to [k+1]$ that extends $f^\adh$ (and $f_S$ on $S \cap \beta(t)$)
and read the best way to extend $f^\beta$ to subgraphs $G[\alpha(s)]$
for $s \in Z$ from the tables $M[s,\cdot,\cdot]$.
To this end, every adhesion $\adh(s)$ fo $s \in Z$ serves as a ``black-box'' that, given 
$f_s^\adh : \adh(s) \to [k+1]$ and requested indices $I_s$, returns minimum cost
that an extension of $f_s^\adh$ to $G_s$ may occur. 
Within the same framework, one can think of edges $e \in E(G_t[\beta(t)])$ as ``mini-black-boxes''
that force us to pay $1$ if $f^\beta$ assigns different values to the endpoints of $e$
and vertices $w \in T_i$ as ``mini-black-boxes'' that allow us to ``score'' the index $i$
if we assign $f^\beta(w) \neq f_S(s_i)$.

This motivates the following definition of a family $\cnstr$ of \emph{constraints};
every child $s \in Z$, every edge $e \in E(G_t[\beta(t)])$, and every pair $(i,w)$, $i \in [t]$, $w \in T_i \cap \beta(t)$ gives rise to a single constraint.
A constraint $\Gamma \in \cnstr$ consists of:
\begin{itemize}
\item a set $X_\Gamma \subseteq \beta(t)$ of size at most $k$;
\item a function $M_\Gamma: 2^{[t]} \times [k+1]^{X_\Gamma} \to \{0,1,2,\ldots,k,+\infty\}$.
\end{itemize}
For a child $s \in Z$, we define a \emph{child constraint} $\Gamma(s)$ as:
\begin{itemize}
\item $X_{\Gamma(s)} = \adh(s)$,
\item $M_{\Gamma(s)}(I_s,f^\adh_s) = M[s,I_s,f^\adh_s]$ for every $I_s \subseteq [t]$ and $f^\adh_s : \adh(s) \to [k+1]$.
\end{itemize}
For an edge $uv = e \in E(G_t[\beta(t)])$, we define an \emph{edge constraint} $\Gamma(e)$ as:
\begin{itemize}
\item $X_{\Gamma(e)} = e$,
\item $M_{\Gamma(e)}(\emptyset, f^\adh_e) = 0$ 
if $f^\adh_e(u) = f^\adh_e(v)$,
 $M_{\Gamma(e)}(\emptyset, f^\adh_e) = 1$ 
if $f^\adh_e(u) \neq f^\adh_e(v)$,
and $M_{\Gamma(e)}(I, f^\adh_e) = +\infty$ for every $I \neq \emptyset$.
\end{itemize}
For a pair $(i,w)$ with $i \in [t]$ and $w \in \beta(t) \cap T_i$ we define a \emph{terminal constraint} $\Gamma(i,w)$ as:
\begin{itemize}
\item $X_{\Gamma(i,w)} = \{w\}$,
\item $M_{\Gamma(i,w)}(\emptyset, \cdot) = 0$, $M_{\Gamma(i,w)}(\{i\},f^\adh_{i,w}) = 0$ if
$f^\adh_{i,w}(w) \neq f_S(s_i)$, and $M_{\Gamma(i,w)}(I, f^\adh_{i,w}) = +\infty$ in all other cases.
\end{itemize}

A \emph{responsibility assignment} is a function $\rho$ that assigns to every constraint $\Gamma \in \cnstr$ a subset $\rho(\Gamma) \subseteq [t]$ such that
the values $\rho(\Gamma)$ are pairwise disjoint over all $\Gamma \in \cnstr$.
For a function $f^\beta : \beta(t) \to [k+1]$ we define the \emph{majority value} $\jmaj(f^\beta)$ as the minimum $j \in [k+1]$ among values $j$
maximizing $|(f^\beta)^{-1}(j)|$ (that is, we take the smallest among the most common values of $f^\beta$).
A function $f^\beta : \beta(t) \to [k+1]$ is \emph{unbreakable-consistent} if either $|\beta(t)| \leq 3k$ or at most $k$ vertices of $\beta(t)$ are assigned values different
than $\jmaj(f^\beta)$.
A \emph{feasible function} is an unbreakable-consistent function $f^\beta : \beta(t) \to [k+1]$ that extents $f^\adh$ on $\adh(t)$ and extends $f_S$ on $S \cap \beta(t)$.

Given a responsibility assignment $\rho$ and a feasible function $f^\beta$, their \emph{cost} is defined as
\begin{equation}\label{eq:mc:cost}
\fcost(\rho,f^\beta) = \sum_{\Gamma \in \cnstr} M_\Gamma(\rho(\Gamma), f^\beta|_{X_\Gamma}).
\end{equation}
We claim the following.
\begin{claim}\label{cl:mc:feas}
Assume that the values $M[s,\cdot,\cdot]$ satisfy Points~\ref{i:mc:cmpl} and~\ref{i:mc:sound} for every $s \in Z$. 
Then the following assignment satisfies Points~\ref{i:mc:cmpl} and~\ref{i:mc:sound} for $t$:
\begin{equation}\label{cl:mc:Mdef}
M[t,I,f^\adh] = \min \{ \fcost(\rho, f^\beta)~|~\rho\mathrm{\ is\ a\ responsibility\ assignment,\ }f^\beta\mathrm{\ is\ a\ feasible\ function,\ }\bigcup_{\Gamma \in \cnstr} \rho(\Gamma) = I \}.
\end{equation}
In the above, $M[t, I, f^\adh] := +\infty$ if the right hand side exceeds $k$.
\end{claim}
\begin{proof}
Let $\rho^\ast$ and $f^{\beta,\ast}$ be values for which the minimum of the right hand side of~\eqref{cl:mc:Mdef} is attained. 

Consider first Point~\ref{i:mc:cmpl} and assume $\rho^\ast$ and $f^{\beta,\ast}$ exist and $\fcost(\rho^\ast, f^{\beta,\ast}) \leq k$. 
In particular, from~\eqref{eq:mc:cost} we infer that for every $\Gamma \in \cnstr$ we have $M_\Gamma(\rho^\ast(\Gamma), f^{\beta,\ast}|_{X_\Gamma}) \leq k$.
For every $s \in Z$ let $f_s$ be the function extending $f^{\beta,\ast}|_{\adh(s)}$ whose existence is promised by Point~\ref{i:mc:cmpl} for the cell
$M_{\Gamma(s)}(\rho^\ast(\Gamma(s)), f^{\beta,\ast}|_{\adh(s)}) \leq k$.
We claim that
$$f := f^{\beta,\ast} \cup \bigcup_{s \in Z} f_s$$
satisfies the requirements for Point~\ref{i:mc:cmpl} for the cell $M[t, I, f^\adh]$.

First, note that $f$ is well-defined as every $f_s$ agrees with $f^{\beta,\ast}$ on $\adh(s)$.
Clearly, $f$ extends $f^\adh$ as $f^{\beta,\ast}$ extends $f^\adh$. Furthermore, as $f^{\beta,\ast}$ and every $f_s$ extends $f_S$ within their domain,
$f$ extends $f_S$ on $V(G_t)$.

Second, fix $i \in I$; are show a vertex $w \in V(G_t)$ for which $f(w) \neq f_S(s_i)$.
By~\eqref{cl:mc:Mdef}, we have $\bigcup_{\Gamma \in \cnstr} \rho^\ast(\Gamma) = I$. 
Hence, there exists $\Gamma_i \in \cnstr$ with $i \in \rho(\Gamma_i)$. 
Since $M_{\Gamma_i}(\rho^\ast(\Gamma_i), f^{\beta,\ast}|_{X_{\Gamma_i}}) \leq k$, $\Gamma_i$ is not an edge constraint $\Gamma(e)$.
If $\Gamma_i$ is a terminal constraint, $\Gamma_i = \Gamma(i,w)$, then from the definition of a terminal constraint we obtain that $f(w) \neq f_S(s_i)$.
Finally, if $\Gamma_i$ is a child contraint, $\Gamma_i = \Gamma(s)$ for some $s \in Z$, then since $f_s$ is a function promised by Point~\ref{i:mc:cmpl} for the cell
$M_{\Gamma(s)}(\rho^\ast(\Gamma(s)), f^{\beta,\ast}|_{\adh(s)})$ there exists $w \in V(G_s)$ with $f_s(w) \neq f_S(s_i)$. 
This concludes the proof that for every $i \in I$ ther exists $w \in V(G_t)$ with $f(w) \neq f_S(s_i)$.

Finally, let us compute the cost of $f$. Let $e = uv \in E(G_t)$ with $f(u) \neq f(v)$. 
By the definition of the graphs $G_t$ and $G_s$, $s \in Z$, $e$ either belongs to $E(G_t[\beta(t)])$ or to exactly one of the subgraphs $G_s$, $s \in Z$.
In the first case, the constraint $\Gamma(e)$ contributes $1$ to $\fcost(\rho^\ast, f^{\beta,\ast})$. 
In the second case, for every $s \in Z$, the number of edges $e = uv \in E(G_s)$ with $f(u) \neq f(v)$ equals exactly the cost of $f_s$, which 
is not larger than $M_{\Gamma(s)}(\rho^\ast(\Gamma(s)), f^{\beta,\ast}_{\adh(s)})$. 
Point~\ref{i:mc:cmpl} for the cell $M[t, I, f^\adh]$ follows.

Let $f$ be a function as in Point~\ref{i:mc:sound} for the cell $M[t, I, f^\adh]$. 
Define responsibility assigment $\rho$ as follows. Start with $\rho(\Gamma) = \emptyset$ for every $\Gamma \in \cnstr$.
For every $i \in I$, proceed as follows. By the properties of Point~\ref{i:mc:sound}, there exists $w_i \in V(G_t)$ with $f(w_i) \neq f_S(s_i)$.
If $w_i \in \beta(t)$, then we insert $i$ into $\rho(\Gamma(i, w_i))$. Otherwise, $w_i \in V(G_s) \setminus \adh(s)$ for some $s \in Z$; we insert then
$i$ into $\rho(\Gamma(s))$. Clearly, $\rho$ is a responsibility assignment and $\bigcup_{\Gamma \in \cnstr} \rho(\Gamma) = I$.

We define $f^\beta = f|_{\beta(t)}$ and we claim that $f^\beta$ is a feasible function. Clearly, $f^\beta$ extends $f^\adh$ and $f_S$ on $\beta(t)$, as $f$ extends
both these functions. To show that $f^\beta$ is unbreakable-consistent, observe that the fact that $\beta(t)$ is $(k,k)$-edge-unbreakable in $G$ with conjunction with the assumption
that the cost of $f$ is at most $k$ implies that for every partition $[t] = I_1 \uplus I_2$ either $(f^\beta)^{-1}(I_1)$ or $(f^\beta)^{-1}(I_2)$ is of size at most $k$.
If $|(f^\beta)^{-1}(\jmaj(f^\beta))| > k$, then this implies that $|(f^\beta)^{-1}([t] \setminus \{\jmaj(f^\beta)\})| \leq k$, as desired.
Otherwise, we have $|(f^\beta)^{-1}(i)| \leq k$ for every $i \in [k+1]$, and unless $|\beta(t)| \leq 3k$ there exist a partition $[t] = I_1 \uplus I_2$ such that
$|(f^\beta)^{-1}(I_j)| > k$ for $j=1,2$, a contradiction. This proves that $f^\beta$ is unbreakable-consistent, and thus a feasible function.

To finish the proof of the claim it suffices to show that for the above defined $\rho$ and $f^\beta$ the cost $\fcost(\rho, f^\beta)$ is at most the cost of $f|_{V(G_t)}$ in $G_t$.
Note that the cost of $f|_{V(G_t)}$ in $G_t$ equals the cost of $f|_{\beta(t)}$ in $G_t[\beta(t)]$ plus the sum over all $s \in Z$ the cost of $f_{V(G_s)}$ in $G_s$.
Consider the types of constraints one by one.

First, consider a child constraint $\Gamma(s)$ for some $s \in Z$. By the definition of $\rho(\Gamma(s))$, $f$ satisfies the requirements for Point~\ref{i:mc:sound}
for the cell $M[s, \rho(\Gamma(s)), f|_{\adh(s)}]$. Consequently, the cost of $f|_{V(G_s)}$ in $G_s$ is not smaller than 
$M[s, \rho(\Gamma(s)), f|_{\adh(s)}] = M_{\Gamma(s)}(\rho(\Gamma(s)), f|_{\adh(s)})$. 
The latter term is exactly the contribution of the constraint $\Gamma(s)$ to the cost $\fcost(\rho,f^\beta)$.

Second, consider an edge $e = uv \in E(G_t[\beta(t)])$. Note that $\rho(\Gamma(e)) = \emptyset$ by definition while $M_{\Gamma(e)}[ \emptyset, f|_e]$ equals $1$
if $f(u) \neq f(v)$ and $0$ otherwise. Thus, the contribution of the edge $e$ towards the cost of $f|_{\beta(t)}$ in $G_t[\beta(t)]$ is the same as the contribution
of $\Gamma(e)$ towards $\fcost(\rho,f^\beta)$.

Third, consider a terminal constraint $\Gamma(i, w)$. If $\rho(\Gamma(i, w)) = \emptyset$, then the contribution of this constraint to $\fcost(\rho,f^\beta)$ is $0$.
Otherwise, we have $\rho(\Gamma(i, w)) = \{i\}$ and this can only happen if $w = w_i$, in particular, $f(w) \neq f_S(s_i)$. 
By definition, this implies $M_{\Gamma(i,w)}(\{i\}, f|_{\{w\}}) = 0$, and again the contribution of this contraint to $\fcost(\rho,f^\beta)$ is $0$.

This concludes the proof that the cost of $f|_{V(G_t)}$ in $G_t$ is not smaller than $\fcost(\rho, f^\beta)$ and concludes the proof of the claim.
\cqed\end{proof}

By Claim~\ref{cl:mc:feas}, it suffices to minimize $\fcost(\rho, f^\beta)$ over responsibility assignments $\rho$ and feasible functions $f^\beta$ such that $\bigcup_{\Gamma \in \cnstr} \rho(\Gamma) = I$.
Assume that this minimum is at most $k$ and fix some minimizing arguments $(\rho^\ast, f^{\beta,\ast})$.
We say that a constraint $\Gamma$ is \emph{touched} if either $\rho^\ast(\Gamma) \neq \emptyset$ or $f^{\beta,\ast}|_{X_\Gamma}$ is not a constant function. We claim the following
\begin{claim}\label{cl:mc:touched}
There are at most $t+k$ touched constraints.
\end{claim}
\begin{proof}
By the assumption that the values $\rho^\ast(\Gamma)$ are pairwise disjoint, there are at most $|I| \leq t$ constraints
with $\rho^\ast(\Gamma) \neq \emptyset$. 
Fix a constraint $\Gamma$ such that $f^{\beta,\ast}|_{X_\Gamma}$ is not a constant function. To finish the proof of the claim
it suffices to show that $\Gamma$ contributes at least $1$ to the sum in~\eqref{eq:mc:cost}. 

Clearly, $\Gamma$ is not a terminal constraint. If $\Gamma$ is an edge constraint, $\Gamma = \Gamma(e)$
for some $e = uv \in E(G_t[\beta(t)])$, then as $X_{\Gamma(e)} = e$ we have $f^{\beta,\ast}(u) \neq f^{\beta,\ast}(v)$.
Hence, $\Gamma$ contributes $1$ to the sum in~\eqref{eq:mc:cost}. 

Finally, if $\Gamma = \Gamma(s)$ for some $s \in Z$, then $\Gamma$ contributes $M[s, \rho(\Gamma(s)), f^{\beta,\ast}|_{\adh(s)}]$
to the sum in~\eqref{eq:mc:cost}. By Point~\ref{i:mc:cmpl}, there exists an extension $f_s$ of $f^{\beta,\ast}_{\adh(s)}$ to $V(G_s)$ of cost at most $M[s,\rho(\Gamma(s)),f^{\beta,\ast}|_{\adh(s)}]$. By $\alpha$-connectivity and the fact that $f^{\beta,\ast}_{\adh(s)}$ is not a constant function, any such extension has a positive cost in $G_s$. This finishes the proof of the claim.
\cqed\end{proof}

Let $A^\ast = (f^{\beta,\ast})^{-1}([k+1] \setminus \{\jmaj(f^{\beta,\ast})\})$. Since $f^{\beta,\ast}$ is unbreakable-consistent, we have $|A^\ast| \leq 3k$. 
Let $B^\ast$ be the set of all vertices $v \in \beta(t) \setminus A^\ast$ for which there exist a touched constraint
$\Gamma \in \cnstr$ with $v \in X_\Gamma$. 
By Claim~\ref{cl:mc:touched}, we have that $|B^\ast| \leq k(k+t)$.

Our application of Lemma~\ref{lem:random2} is encapsulated in the following claim.
\begin{claim}\label{cl:mc:random}
In time $2^{\Oh((k+t) \log (k+t))} n^{\Oh(1)}$ one can generate a family $\randfamily$
of pairs $(j,g)$ where $j \in [k+1]$ and $g : \beta(t) \to [k+1]$.
The family is of size $2^{\Oh((k+t) \log (k+t))} n$ and
there exists $(j,g) \in \randfamily$ such that $j = \jmaj(f^{\beta,\ast})$ and $g$ agrees with $f^{\beta,\ast}$ on
$A^\ast \cup B^\ast$. Furthermore, for every element $(j,g) \in \randfamily$, $g$ agrees with $f^{\beta,\ast}$
on $\adh(t) \cup (S \cap \beta(t))$. 
\end{claim}
\begin{proof}
Let $S' = (S \cap \beta(t)) \cup \adh(t)$. 

First, we iterate over all choices of nonnegative integers $j \in [k+1]$ and $a_1,a_2, \ldots, a_{k+1}$
such that $\sum_{i=1}^{k+1} a_i \leq 3k+k(k+t)$ and $\sum_{i \in [k+1] \setminus \{j\}} a_i \leq 3k$. 
Clearly, there are $2^{\Oh(k)}$ options.
For a fixed choice of $j$ and $(a_i)_{i=1}^{k+1}$ we invoke Lemma~\ref{lem:random2}
for $U = \beta(t) \setminus S'$ and integers $r = k+1$, $(a_i)_{i=1}^{k+1}$, obtaining a family
$\randfamily'$. For every $g' \in \randfamily'$, we insert $(j, g' \cup f^\adh|_{\adh(t)} \cup f_S|_{S \cap \beta(t)})$
  into $\randfamily$.

The bound on the size of the output family $\randfamily$ follows from bound of Lemma~\ref{lem:random2}
and the inequality $log^k n \leq 2^{\Oh(k \log k)} n$. 
Finally, note that the promised pair $(j,g)$ will be generated for the choice of
$j = \jmaj(f^{\beta,\ast})$ and $a_i = |(f^{\beta,\ast})^{-1}(i) \cap (A^\ast \cup B^\ast)|$ for every $i \in [k+1]$.
\cqed\end{proof}

Invoke the algorithm of Claim~\ref{cl:mc:random}, obtaining a family $\randfamily$. We say
that $(j,g) \in \randfamily$ is \emph{lucky} if $f^{\beta,\ast}$ exists, $j = \jmaj(f^{\beta,\ast})$, and $f^{\beta,\ast}$
agrees with $g$ on $A^\ast \cup B^\ast$. 

Consider now an auxiliary graph $H$ with $V(H) = \beta(t)$ and $uv \in E(H)$ if and only if
$u \neq v$ and there exists a constraint $\Gamma \in \cnstr$ with $u,v\in X_\Gamma$.
By the definition of constraints $\Gamma(e)$, we have that $G_t[\beta(t)]$ is a subgraph of
$H$, but in $H$ we also turn all adhesions $\adh(s)$ for $s \in Z$ into cliques.

For a pair $(j,g) \in \randfamily$, we define $\Sigma(j,g) := g^{-1}([k+1] \setminus \{j\})$.
Observe the following.

\begin{claim}\label{cl:mc:stains}
For a lucky pair $(j,g)$,
every connected component of $H[\Sigma(j,g)]$ is either completely contained
in $(f^{\beta,\ast})^{-1}(j)$ or completely contained in $A^\ast$.
\end{claim}
\begin{proof}
Assume the contrary, and let $uv \in E(H)$ be an edge violating the condition. By symmetry, assume $f^{\beta,\ast}(u) \neq j$.
Then, since $(j,g)$ is lucky, we have that $u \in A^\ast$. Hence $v \notin A^\ast$, that is, $f^{\beta,\ast}(v) = j$. 
By the definition of $H$, there exists a constraint $\Gamma \in \cnstr$ with $u,v \in X_{\Gamma}$ (either $\Gamma = \Gamma(uv)$ or
$\Gamma = \Gamma(s)$ for some $s \in Z$ with $u,v \in \adh(s)$). Consequently, $\Gamma$ is touched, and $v \in B^\ast$.
However, then from the fact that $(j,g)$ is lucky it follows that $g(v) = j$, a contradiction.
\cqed\end{proof}
Claim~\ref{cl:mc:stains} motivates the following approach. We try every pair $(j,g) \in \randfamily$,
and proceed under the assumption that $(j,g)$ is lucky. 
We inspect connected components of $H[\Sigma(j,g)]$ one-by-one and either try to 
set a candidate for function $f^{\beta,\ast}$ to be equal to $g$ or constantly equal $j$ on the component.
Claim~\ref{cl:mc:stains} asserts that one could construct $f^{\beta,\ast}$.
The definition of $H$ implies that for every constraint $\Gamma \in \cnstr$, the set $X_\Gamma$ intersects at most one component
of $H[\Sigma(j,g)]$. This gives significant
independence of the decisions, allowing us to execute a multidimensional knapsack-type dynamic
programming, as between different connected components of $H[\Sigma(j,g)]$ we need only to keep intermediate values of the
cost and the union of values of the constructed responsibility assignment. 

We proceed with formal arguments. 
For every $(j,g) \in \randfamily$, we proceed as follows.
Let $C_1,C_2,\ldots,C_\ell$ be the connected components of $H[\Sigma(j,g)]$ and for $1 \leq i \leq \ell$, 
let $\cnstr_i$ be the set of constraints $\Gamma \in \cnstr_i$ with
$X_\Gamma \cap C_i \neq \emptyset$.
By the definition of $H$,
  the sets $\cnstr_i$ are pairwise disjoint.
Let $\cnstr_0 = \cnstr \setminus \bigcup_{i=1}^\ell \cnstr_i$ be the remaining constraints, i.e., the constraints $\Gamma \in \cnstr$ with $X_\Gamma \cap \Sigma(j,g) = \emptyset$.
It will be convenient for us to denote $C_0 = \emptyset$ to be a component accompanying
$\cnstr_0$.
For $J \subseteq \{0,1,2,\ldots,\ell\}$, denote $g_J$ to be the function $g$ modified as follows: 
for every $i \in \{0,1,\ldots,\ell\} \setminus J$ and every $v \in C_i$ we set $g_J(v) = j$.
Furthermore, let $J^\adh \subseteq \{1,2,\ldots,\ell\}$ be the set of these indices $j$
for which $C_j \cap (\adh(t) \cup S) \neq \emptyset$.
For $0 \leq i \leq \ell$, denote $\cnstr_{\leq i} = \bigcup_{j \leq i} \cnstr_j$.

Let $m = |\cnstr|$. We order constraints in $\cnstr$ as $\Gamma_1,\Gamma_2,\ldots,\Gamma_m$
according to which set $\cnstr_i$ they belong to. That is, if $\Gamma_a \in \cnstr_i$,
$\Gamma_b \in \cnstr_j$ and $i < j$, then $a < b$.
For $0 \leq i \leq \ell$,
let $\lasta(i) = |\cnstr_{\leq i}|$, that is, $\Gamma_{\lasta(i)} \in \cnstr_{\leq i}$
but $\Gamma_{\lasta(i)+1}$ does not belong to $\cnstr_{\leq i}$ (if exists).
Furthermore, let $\lasta(-1) = 0$.
In the reverse direction, for $1 \leq a \leq m$, let $\geti(a) \in \{0,1,\ldots,\ell\}$
be such that $\Gamma_a \in \cnstr_{\geti(a)}$.

Let $0 \leq i \leq \ell$ and let $\lasta(i-1) \leq a \leq \lasta(i)$.
A \emph{$a$-partial responsibility assignment} $\rho$ is a responsibility assignment
defined on constraints $\Gamma_1, \ldots, \Gamma_a$ such that $\bigcup_{b=1}^a \rho(\Gamma_b) \subseteq I$.
For a set $J \subseteq \{0,1,\ldots,i\}$ containing $J^\adh \cap \{0,1,\ldots,i\}$
and an $a$-partial responsibility assignment $\rho$, we define the cost of $J$ and $a$ as
$$\fcost_{i,a}(J, \rho) = \sum_{b=1}^a M_{\Gamma_b}(\rho(\Gamma_b), g_J|_{X_{\Gamma_b}}).$$
Furthermore, let $k^\beta = k$ if $|\beta(t)| > 3k$ and $k^\beta = |\beta(t)|$ otherwise.
The goal of our dynamic programming algorithm is to compute, for every $-1 \leq i \leq \ell$, $0 \leq k^\bullet \leq k^\beta$,
 and $I^\bullet \subseteq I$
a value $Q_i[k^\bullet, I^\bullet]$ that equals a minimum possible cost $\fcost_{i,\lasta(i)}(J,\rho)$ over all $J \subseteq \{0,1,\ldots,i\}$ containing $J^\adh \cap \{0,1,\ldots,i\}$ with $|\bigcup_{i' \in J} C_{i'}| \leq k^\bullet$,
and $\lasta(i)$-partial responsibility assignment $\rho$
with $\bigcup_{b=1}^{\lasta(i)} \rho(\Gamma_b) = I^\bullet$.
The next claim shows that it suffices.
\begin{claim}\label{cl:mc:dp}
We have $Q_\ell[k^\beta, I] \geq \fcost(\rho^\ast, f^{\beta,\ast})$. 
Furthermore, if $\fcost(\rho^\ast,f^{\beta,\ast}) \leq k$ and $(j,g)$ is lucky, then 
$Q_\ell[k^\beta,I] = \fcost(\rho^\ast, f^{\beta,\ast})$.
\end{claim}
\begin{proof}
For the first claim, let $(J, \rho)$ be the witnessing arguments for the calue $Q_\ell[k^\beta, I]$.
Note that $\rho$ is a responsibility assignment. Furthermore, $g_J$ is a feasible function: it extends $f^\adh$
and $f_S$ on $S \cap \beta(t)$ due to the requirement $J^\adh \subseteq J$ and it is unbreakable-consistent
due to the requirement $|\bigcup_{i' \in J} C_{i'}| \leq k^\beta$. 
The first claim follows from the minimality of $(\rho^\ast, f^{\beta,\ast})$.

For the second claim, by Claim~\ref{cl:mc:stains} we know that on every connected component $C_i$,
the function $f^{\beta,\ast}$ either equals $g$ or is constant at $j$. 
Let $J^\ast$ be the set where the first option happens; note that $J^\adh \subseteq J^\ast$
and $g_{J^\ast} = f^{\beta,\ast}$. Consequently, $\fcost_{\ell,m}(J^\ast, \rho^\ast) = \fcost(\rho^\ast, f^{\beta,\ast})$. 
Finally, as $f^{\beta,\ast}$ is unbreakable-consistent, we have $|\bigcup_{i' \in J^\ast} C_{i'}| \leq k^\beta$.
The claim follows from the minimality of $Q_\ell[k^\beta, I]$.
\cqed\end{proof}

For the initialization step of our dynamic programming algorithm, note that for $i=-1$
we have $\lasta(i)=0$ and the minimization for $Q_{-1}[\cdot,\cdot]$
takes into account only $J = \emptyset$ and $\rho=\emptyset$.

Fix now $0 \leq i \leq \ell$, we are to compute values $Q_i[\cdot,\cdot]$. 
To this end, we use another layer of dynamic programming.
For $\lasta(i-1) \leq a \leq \lasta(i)$, $0 \leq k^\bullet \leq k^\beta$, and $I^\bullet \subseteq I$
we define $Q_{i,a}^\in[k^\bullet, I^\bullet]$ to be a minimum possible cost
$\fcost_{i,a}(\rho,J)$ over all $J \subseteq \{0,1,2,\ldots,i\}$ containing
$J^\adh \cap \{0,1,2,\ldots,i\}$ and the index $i$ with the property that
$|\bigcup_{i' \in J} C_{i'}| \leq k^\bullet$, and all $a$-partial responsibility assigments
$\rho$ with $\bigcup_{b=1}^a \rho(\Gamma_b) = I^\bullet$.

Similarly we define $Q_{i,a}^{\notin}[k^\bullet, I^\bullet]$ with the requirement that $i \notin J$.
This definition is applicable only if $i \notin J^\adh$; for indices $i \in J^\adh$ we do not compute
values $Q_{i,a}^{\notin}$.

Since $Q_{i,\lasta(i-1)}^\in$, $Q_{i,\lasta(i-1)}^{\notin}$, and $Q_{i-1}$ use all constraints up to $\lasta(i-1)$,
we have
$$Q_{i,\lasta(i-1)}^\in[k^\beta + |C_i|, I^\bullet] = Q_{i,\lasta(i-1)}^{\notin}[k^\beta, I^\bullet] = Q_{i-1}[k^\beta, I^\bullet].$$
Here, and in subsequent formulae, we assume that a value of a cell $Q_{i,a}^\in[\cdot,\cdot]$
or $Q_i[\cdot,\cdot]$ equals $0$ if the argument is negative.
The above formula serves as the initialization step for computing values $Q_{i,a}^\in[\cdot,\cdot]$
and $Q_{i,a}^\in[\cdot,\cdot]$.

For a single computation step, fix $\lasta(i-1) < a \leq \lasta(i)$.
The definitions of $Q_{i,a}^\in[\cdot]$ and $Q_{i,a-1}^\in[\cdot,\cdot]$ differ only in the requirement
to define $f(\Gamma_a)$. Furthermore, $X_{\Gamma_a}$ intersects only the component $C_i$
(if $i > 0$), while $i$ is required to be contained in $J$ in the definition
of both $Q_{i,a}^\in[\cdot,\cdot]$ and $Q_{i,a-1}^\in[\cdot,\cdot]$. Consequently,
$$Q_{i,a}^\in[k^\bullet, I^\bullet] = \min_{I' \subseteq I^\bullet} \left(Q_{i,a-1}^\in[k^\bullet, I^\bullet \setminus I'] + M_{\Gamma_a}(I', g|_{X_{\Gamma_a}})\right).$$
  Similarly, for $i \notin J^\adh$ we have  
$$Q_{i,a}^\in[k^\bullet, I^\bullet] = \min_{I' \subseteq I^\bullet} \left(Q_{i,a-1}^\in[k^\bullet, I^\bullet \setminus I'] + M_{\Gamma_a}(I', X_{\Gamma_a} \times \{j\})\right).$$
  Finally, we set for $i \in J^\adh$:
$$Q_i[k^\bullet, I^\bullet] = Q_{i,\lasta(i)}[k^\bullet, I^\bullet],$$
and for $i \notin J^\adh$:
$$Q_i[k^\bullet, I^\bullet] = \min \left( Q_{i,\lasta(i)}^\in[k^\bullet, I^\bullet], Q_{i,\lasta(i)}^{\notin}[k^\bullet, I^\bullet]\right)$$

The above dynamic programming algorithm computes the values $Q_\ell[\cdot]$ in time $3^t \cdot n^{\Oh(1)}$.
By Claims~\ref{cl:mc:feas} and~\ref{cl:mc:dp}, we can take $M[t, I, f^\adh]$
to be the minimum value of $Q_\ell[k^\beta, I]$ encountered over all choices of $(j,g) \in \randfamily$.
Claim~\ref{cl:mc:M} shows that the above suffices to conclude the proof of Theorem~\ref{thm:multicut}.
\end{proof}




==> algo-steinercut.tex <==
We now apply the framework to the \textsc{Steiner Cut} problem.
In this problem we are given an undirected graph $G$, a set $T \subseteq V(G)$ of terminals, and integers $k,p$. 
The goal is to delete at most $k$ edges from $G$ so that $G$ has at least $p$ connected components containing
at least one terminal.

Kawarabayashi and Thorup~\cite{KT11} showed a first FPT algorithm for \textsc{Steiner Cut} in the variant $V(G) = T$,
and Chitnis et al.~\cite{randcontr} improved the running time and generalized to the case of general $T$.
We use our decomposition theorem to further improve the exponential part of the running time bound.
\begin{theorem}\label{thm:steinercut}
\textsc{Steiner Cut} can be solved in time $2^{\Oh(k \log k)} n^{\Oh(1)}$.
\end{theorem}

\begin{proof}
Let $(G,T,p,k)$ be an input to \textsc{Steiner Cut} and let $n = |V(G)|$. 

First, we observe that it is sufficient to solve \textsc{Steiner Cut} with the additional assumption that $G$ is connected.
Indeed, in the general case we can proceed as follows. First, we discard all connected components of $G$
that are disjoint with $T$. 
Second, for every connected component $G'$ of $G$ and every $0 \leq k' \leq k$, $0 \leq p' \leq p$, we solve \textsc{Steiner Cut}
on the instance $(G', T \cap V(G'), p', k')$.
Finally, the results of these computations allow us to solve the input instance by a straightforward knapsack-type
dynamic programming algorithm.
Thus, henceforth we assume that $G$ is connected. In particular, we can assume that $p \leq k+1$ as otherwise the input
instance is a trivial no-instance.

Assume we are given a graph $H$ and a function $f : V(H) \to [p]$.
The \emph{cost} of $f$ on $H$
is defined as the number of edges $uv \in E(H)$ with $f(u) \neq f(v)$
and denoted as $\fcost_H(f)$.
Since $G$ is connected, the \textsc{Steiner Cut} problem on $(G,T,p,k)$ can be reformulated in the following way:
does there exist $f : V(G) \to [p]$ of cost at most $k$ such that $f(T) = [p]$?
We henceforth refer to such $f$ as a \emph{solution}.

We invoke the algorithm of Theorem~\ref{thm:decomp} to $G$ and $k$,
obtaining a rooted compact
tree decomposition $(T,\beta)$ of $G$ whose every bag is $(k,k)$-edge-unbreakable
and every adhesion is of size at most $k$. The running time of this step 
is $2^{\Oh(k \log k)} n^{\Oh(1)}$.

We perform a bottom-up dynamic programming algorithm on $(T,\beta)$. 
For every node $t \in V(T)$, every subset $I \subseteq [p]$, and every
function $f^\adh: \adh(t) \to [p]$,  we compute a value $M[t, I, f^\adh] \in \{0, 1, 2, \ldots, k, +\infty\}$
with the following properties.

\begin{enumerate}[label={(\alph*)}]
\item If $M[t,I, f^\adh] \neq +\infty$, then there exists a function $f : V(G_t) \to [p]$ such that:\label{i:sc:cmpl}
\begin{itemize}
\item $f|_{\adh(t)} = f^\adh$,
\item for every $i \in I$ there exists $w_i \in V(G_t) \cap T$ with $f(w_i) = i$,
\item the cost of $f$ in $G_t$ is at most $M[t,I,f^\adh]$.
\end{itemize}
\item For every function $f : V(G) \to [p]$ that satisfies:\label{i:sc:sound}
\begin{itemize}
\item $f|_{\adh(t)} = f^\adh$,
\item for every $i \in [p]$ there exists $w_i \in T$ with $f(w_i) = i$, and, 
  furthermore, if $i \in I$ there exists $w_i \in T \cap V(G_t)$ with $f(w_i) = i$,
\item the cost of $f$ in $G$ is at most $k$,
\end{itemize}
the cost of $f|_{V(G_t)}$ in $G_t$ is at least $M[t,I,f^\adh]$.
\end{enumerate}

We first observe that the table $M[\cdot]$ is sufficient for our purposes.
\begin{claim}\label{cl:sc:M}
There exists a solution if and only if
$M[r,[t],\emptyset] \neq +\infty$ for the root $r$ of $T$.
\end{claim}
\begin{proof}
In one direction, if $f$ is a solution, then note that
$f$ satisfies all conditions of Point~\ref{i:sc:sound} for the cell
$M[r,[t],\emptyset]$. Hence, by Point~\ref{i:sc:sound}, $M[r,[t],\emptyset] < +\infty$.

In the other direction, let $M[r,[t],\emptyset] < +\infty$ and 
let $f$ be the function whose existence is asserted by Point~\ref{i:sc:cmpl}.
Then for every $i \in [t]$ there exists $w_i \in T$ with $f(w_i) = i$ and its cost in $G_r = G$ is at most $k$.
Consequently, $f$ is a solution.
\cqed\end{proof}

Thus, to prove Theorem~\ref{thm:steinercut}, it suffices to show now to compute in time $2^{\Oh(k \log k)} n^{\Oh(1)}$
entries $M[t,\cdot,\cdot]$ for a fixed note $t \in V(T)$, given entries $M[s,\cdot,\cdot]$ for all children $s$ of $t$ in $T$.
Since $|\adh(t)| \leq k$ and $p \leq k+1$, it suffices to focus on a computation of a single cell $M[t,I,f^\adh]$. 
Let $Z$ be the set of children of $t$ in $T$.

In a single step of a dynamic programming algorith, we would like to focus on finding
a function $f^\beta : \beta(t) \to [p]$ that extends $f^\adh$
and read the best way to extend $f^\beta$ to subgraphs $G[\alpha(s)]$
for $s \in Z$ from the tables $M[s,\cdot,\cdot]$.
To this end, every adhesion $\adh(s)$ for $s \in Z$ serves as a ``black-box'' that, given 
$f_s^\adh : \adh(s) \to [p]$ and requested indices $I_s$, returns minimum cost
that an extension of $f_s^\adh$ to $G_s$ may occur. 
Within the same framework, one can think of edges $e \in E(G_t[\beta(t)])$ as ``mini-black-boxes''
that force us to pay $1$ if $f^\beta$ assigns different values to the endpoints of $e$
and vertices $w \in T$ as ``mini-black-boxes'' that allow us to ``score'' the index $i$
if we assign $f^\beta(w) = i$.

This motivates the following definition of a family $\cnstr$ of \emph{constraints};
every child $s \in Z$, every edge $e \in E(G_t[\beta(t)])$, and every vertex $w \in T \cap \beta(t)$
gives raise to a single constraint.
A constraint $\Gamma \in \cnstr$ consists of:
\begin{itemize}
\item a set $X_\Gamma \subseteq \beta(t)$ of size at most $k$;
\item a function $M_\Gamma: 2^{[t]} \times [p]^{X_\Gamma} \to \{0,1,2,\ldots,k,+\infty\}$.
\end{itemize}
For a child $s \in Z$, we define a \emph{child constraint} $\Gamma(s)$ as:
\begin{itemize}
\item $X_{\Gamma(s)} = \adh(s)$,
\item $M_{\Gamma(s)}(I_s,f^\adh_s) = M[s,I_s,f^\adh_s]$ for every $I_s \subseteq [p]$ and $f^\adh_s : \adh(s) \to [p]$.
\end{itemize}
For an edge $uv = e \in E(G_t[\beta(t)])$, we define an \emph{edge constraint} $\Gamma(e)$ as:
\begin{itemize}
\item $X_{\Gamma(e)} = e$,
\item $M_{\Gamma(e)}(\emptyset, f^\adh_e) = 0$ 
if $f^\adh_e(u) = f^\adh_e(v)$,
 $M_{\Gamma(e)}(\emptyset, f^\adh_e) = 1$ 
if $f^\adh_e(u) \neq f^\adh_e(v)$,
and $M_{\Gamma(e)}(I, f^\adh_e) = +\infty$ for every $I \neq \emptyset$.
\end{itemize}
For a vertex $w \in T \cap \beta(t)$ we define a \emph{terminal constraint} $\Gamma(w)$ as:
\begin{itemize}
\item $X_{\Gamma(w)} = \{w\}$,
\item $M_{\Gamma(w)}(\emptyset, \cdot) = 0$, $M_{\Gamma(w)}(\{i\},f^\adh_{w}) = 0$ if
$f^\adh_{w}(w) = i$, and $M_{\Gamma(w)}(I, f^\adh_{w}) = +\infty$ in all other cases.
\end{itemize}
A \emph{responsibility assignment} is a function $\rho$ that assigns to every constraint $\Gamma \in \cnstr$ a subset $\rho(\Gamma) \subseteq [p]$ such that
the values $\rho(\Gamma)$ are pairwise disjoint over all $\Gamma \in \cnstr$.
For a function $f^\beta : \beta(t) \to [p]$ we define the \emph{majority value} $\jmaj(f^\beta)$ as the minimum $j \in [p]$ among values $j$
maximizing $|(f^\beta)^{-1}(j)|$ (that is, we take the smallest among the most common values of $f^\beta$).
A function $f^\beta : \beta(t) \to [p]$ is \emph{unbreakable-consistent} if either $|\beta(t)| \leq 3k$ or at most $k$ vertices of $\beta(t)$ are assigned values different
than $\jmaj(f^\beta)$.
A \emph{feasible function} is an unbreakable-consistent function $f^\beta : \beta(t) \to [p]$ that extents $f^\adh$ on $\adh(t)$.

Given a responsibility assignment $\rho$ and a feasible function $f^\beta$, their \emph{cost} is defined as
\begin{equation}\label{eq:sc:cost}
\fcost(\rho,f^\beta) = \sum_{\Gamma \in \cnstr} M_\Gamma(\rho(\Gamma), f^\beta|_{X_\Gamma}).
\end{equation}
We claim the following.
\begin{claim}\label{cl:sc:feas}
Assume that the values $M[s,\cdot,\cdot]$ satisfy Points~\ref{i:sc:cmpl} and~\ref{i:sc:sound} for every $s \in Z$. 
Then the following assignment satisfies Points~\ref{i:sc:cmpl} and~\ref{i:sc:sound} for $t$:
\begin{equation}\label{cl:sc:Mdef}
M[t,I,f^\adh] = \min \{ \fcost(\rho, f^\beta)~|~\rho\mathrm{\ is\ a\ responsibility\ assignment,\ }f^\beta\mathrm{\ is\ a\ feasible\ function,\ }\bigcup_{\Gamma \in \cnstr} \rho(\Gamma) = I \}.
\end{equation}
In the above, $M[t, I, f^\adh] := +\infty$ if the right hand side exceeds $k$.
\end{claim}
\begin{proof}
Let $\rho^\ast$ and $f^{\beta,\ast}$ be values for which the minimum of the right hand side of~\eqref{cl:sc:Mdef} is attained. 

Consider first Point~\ref{i:sc:cmpl} and assume $\rho^\ast$ and $f^{\beta,\ast}$ exist and $\fcost(\rho^\ast, f^{\beta,\ast}) \leq k$. 
In particular, from~\eqref{eq:sc:cost} we infer that for every $\Gamma \in \cnstr$ we have $M_\Gamma(\rho^\ast(\Gamma), f^{\beta,\ast}|_{X_\Gamma}) \leq k$.
For every $s \in Z$ let $f_s$ be the function extending $f^{\beta,\ast}|_{\adh(s)}$ whose existence is promised by Point~\ref{i:sc:cmpl} for the cell
$M_{\Gamma(s)}(\rho^\ast(\Gamma(s)), f^{\beta,\ast}|_{\adh(s)}) \leq k$.
We claim that
$$f := f^{\beta,\ast} \cup \bigcup_{s \in Z} f_s$$
satisfies the requirements for Point~\ref{i:sc:cmpl} for the cell $M[t, I, f^\adh]$.

First, note that $f$ is well-defined as every $f_s$ agrees with $f^{\beta,\ast}$ on $\adh(s)$.
Clearly, $f$ extends $f^\adh$ as $f^{\beta,\ast}$ extends $f^\adh$.

Second, fix $i \in I$; are show a vertex $w \in T \cap V(G_t)$ for which $f(w) = i$.
By~\eqref{cl:sc:Mdef}, we have $\bigcup_{\Gamma \in \cnstr} \rho^\ast(\Gamma) = I$. 
Hence, there exists $\Gamma_i \in \cnstr$ with $i \in \rho(\Gamma_i)$. 
Since $M_{\Gamma_i}(\rho^\ast(\Gamma_i), f^{\beta,\ast}|_{X_{\Gamma_i}}) \leq k$, $\Gamma_i$ is not an edge constraint $\Gamma(e)$.
If $\Gamma_i$ is a terminal constraint, $\Gamma_i = \Gamma(w)$, then from the definition of a terminal constraint we obtain that $f(w) = i$.
Finally, if $\Gamma_i$ is a child contraint, $\Gamma_i = \Gamma(s)$ for some $s \in Z$, then since $f_s$ is a function promised by Point~\ref{i:sc:cmpl} for the cell
$M_{\Gamma(s)}(\rho^\ast(\Gamma(s)), f^{\beta,\ast}|_{\adh(s)})$ there exists $w \in V(G_s) \cap T$ with $f_s(w) = i$.
This concludes the proof that for every $i \in I$ ther exists $w \in V(G_t) \cap T$ with $f(w) = i$.

Finally, let us compute the cost of $f$. Let $e = uv \in E(G_t)$ with $f(u) \neq f(v)$. 
By the definition of the graphs $G_t$ and $G_s$, $s \in Z$, $e$ either belongs to $E(G_t[\beta(t)])$ or to exactly one of the subgraphs $G_s$, $s \in Z$.
In the first case, the constraint $\Gamma(e)$ contributes $1$ to $\fcost(\rho^\ast, f^{\beta,\ast})$. 
In the second case, for every $s \in Z$, the number of edges $e = uv \in E(G_s)$ with $f(u) \neq f(v)$ equals exactly the cost of $f_s$, which 
is not larger than $M_{\Gamma(s)}(\rho^\ast(\Gamma(s)), f^{\beta,\ast}_{\adh(s)})$. 
Point~\ref{i:sc:cmpl} for the cell $M[t, I, f^\adh]$ follows.

Let $f$ be a function as in Point~\ref{i:sc:sound} for the cell $M[t, I, f^\adh]$. 
Define responsibility assigment $\rho$ as follows. Start with $\rho(\Gamma) = \emptyset$ for every $\Gamma \in \cnstr$.
For every $i \in I$, proceed as follows. By the properties of Point~\ref{i:sc:sound}, there exists $w \in V(G_t) \cap T$ with $f(w) = i$.
If $w \in \beta(t)$, then we insert $i$ into $\rho(\Gamma(w)))$. Otherwise, $w \in V(G_s) \setminus \adh(s)$ for some $s \in Z$; we insert then
$i$ into $\rho(\Gamma(s))$. Clearly, $\rho$ is a responsibility assignment and $\bigcup_{\Gamma \in \cnstr} \rho(\Gamma) = I$.

We define $f^\beta = f|_{\beta(t)}$ and we claim that $f^\beta$ is a feasible function. Clearly, $f^\beta$ extends $f^\adh$.
To show that $f^\beta$ is unbreakable-consistent, observe that the fact that $\beta(t)$ is $(k,k)$-edge-unbreakable in $G$ with conjunction with the assumption
that the cost of $f$ is at most $k$ implies that for every partition $[p] = I_1 \uplus I_2$ either $(f^\beta)^{-1}(I_1)$ or $(f^\beta)^{-1}(I_2)$ is of size at most $k$.
If $|(f^\beta)^{-1}(\jmaj(f^\beta))| > k$, then this implies that $|(f^\beta)^{-1}([p] \setminus \{\jmaj(f^\beta)\})| \leq k$, as desired.
Otherwise, we have $|(f^\beta)^{-1}(i)| \leq k$ for every $i \in [p]$, and unless $|\beta(t)| \leq 3k$ there exist a partition $[p] = I_1 \uplus I_2$ such that
$|(f^\beta)^{-1}(I_j)| > k$ for $j=1,2$, a contradiction. This proves that $f^\beta$ is unbreakable-consistent, and thus a feasible function.

To finish the proof of the claim it suffices to show that for the above defined $\rho$ and $f^\beta$ the cost $\fcost(\rho, f^\beta)$ is at most the cost of $f|_{V(G_t)}$ in $G_t$.
Note that the cost of $f|_{V(G_t)}$ in $G_t$ equals the cost of $f|_{\beta(t)}$ in $G_t[\beta(t)]$ plus the sum over all $s \in Z$ the cost of $f_{V(G_s)}$ in $G_s$.
Consider the types of constraints one by one.

First, consider a child constraint $\Gamma(s)$ for some $s \in Z$. By the definition of $\rho(\Gamma(s))$, $f$ satisfies the requirements for Point~\ref{i:sc:sound}
for the cell $M[s, \rho(\Gamma(s)), f|_{\adh(s)}]$. Consequently, the cost of $f|_{V(G_s)}$ in $G_s$ is not smaller than 
$M[s, \rho(\Gamma(s)), f|_{\adh(s)}] = M_{\Gamma(s)}(\rho(\Gamma(s)), f|_{\adh(s)})$. 
The latter term is exactly the contribution of the constraint $\Gamma(s)$ to the cost $\fcost(\rho,f^\beta)$.

Second, consider an edge $e = uv \in E(G_t[\beta(t)])$. Note that $\rho(\Gamma(e)) = \emptyset$ by definition while $M_{\Gamma(e)}[ \emptyset, f|_e]$ equals $1$
if $f(u) \neq f(v)$ and $0$ otherwise. Thus, the contribution of the edge $e$ towards the cost of $f|_{\beta(t)}$ in $G_t[\beta(t)]$ is the same as the contribution
of $\Gamma(e)$ towards $\fcost(\rho,f^\beta)$.

Third, consider a terminal constraint $\Gamma(w)$. If $\rho(\Gamma(w)) = \emptyset$, then the contribution of this constraint to $\fcost(\rho,f^\beta)$ is $0$.
Otherwise, we have $\rho(\Gamma(w)) = \{f(w)\}$.
By definition, this implies $M_{\Gamma(i,w)}(\{i\}, f|_{\{w\}}) = 0$, and again the contribution of this contraint to $\fcost(\rho,f^\beta)$ is $0$.

This concludes the proof that the cost of $f|_{V(G_t)}$ in $G_t$ is not smaller than $\fcost(\rho, f^\beta)$ and concludes the proof of the claim.
\cqed\end{proof}

By Claim~\ref{cl:sc:feas}, it suffices to minimize $\fcost(\rho, f^\beta)$ over responsibility assignments $\rho$ and feasible functions $f^\beta$ such that $\bigcup_{\Gamma \in \cnstr} \rho(\Gamma) = I$.
Assume that this minimum is at most $k$ and fix some minimizing arguments $(\rho^\ast, f^{\beta,\ast})$.
We say that a constraint $\Gamma$ is \emph{touched} if either $\rho^\ast(\Gamma) \neq \emptyset$ or $f^{\beta,\ast}|_{X_\Gamma}$ is not a constant function. We claim the following
\begin{claim}\label{cl:sc:touched}
There are at most $p+k \leq 2k+1$ touched constraints.
\end{claim}
\begin{proof}
By the assumption that the values $\rho^\ast(\Gamma)$ are pairwise disjoint, there are at most $|I| \leq p$ constraints
with $\rho^\ast(\Gamma) \neq \emptyset$. 
Fix a constraint $\Gamma$ such that $f^{\beta,\ast}|_{X_\Gamma}$ is not a constant function. To finish the proof of the claim
it suffices to show that $\Gamma$ contributes at least $1$ to the sum in~\eqref{eq:sc:cost}. 

Clearly, $\Gamma$ is not a terminal constraint. If $\Gamma$ is an edge constraint, $\Gamma = \Gamma(e)$
for some $e = uv \in E(G_t[\beta(t)])$, then as $X_{\Gamma(e)} = e$ we have $f^{\beta,\ast}(u) \neq f^{\beta,\ast}(v)$.
Hence, $\Gamma$ contributes $1$ to the sum in~\eqref{eq:sc:cost}. 

Finally, if $\Gamma = \Gamma(s)$ for some $s \in Z$, then $\Gamma$ contributes $M[s, \rho(\Gamma(s)), f^{\beta,\ast}|_{\adh(s)}]$
to the sum in~\eqref{eq:sc:cost}. By Point~\ref{i:sc:cmpl}, there exists an extension $f_s$ of $f^{\beta,\ast}_{\adh(s)}$ to $V(G_s)$ of cost at most $M[s,\rho(\Gamma(s)),f^{\beta,\ast}|_{\adh(s)}]$. By $\alpha$-connectivity and the fact that $f^{\beta,\ast}_{\adh(s)}$ is not a constant function, any such extension has a positive cost in $G_s$. This finishes the proof of the claim.
\cqed\end{proof}

Let $A^\ast = (f^{\beta,\ast})^{-1}([p] \setminus \{\jmaj(f^{\beta,\ast})\})$.
Since $f^{\beta,\ast}$ is unbreakable-consistent, we have $|A^\ast| \leq 3k$. 
Let $B^\ast$ be the set of all vertices $v \in \beta(t) \setminus A^\ast$ for which there exist a touched constraint
$\Gamma \in \cnstr$ with $v \in X_\Gamma$. 
By Claim~\ref{cl:sc:touched}, we have that $|B^\ast| \leq k(k+p) = \Oh(k^2)$.

Our application of Lemma~\ref{lem:random2} is encapsulated in the following claim.
\begin{claim}\label{cl:sc:random}
In time $2^{\Oh(k \log k)} n^{\Oh(1)}$ one can generate a family $\randfamily$
of pairs $(j,g)$ where $j \in [p]$ and $g : \beta(t) \to [p]$.
The family is of size $2^{\Oh(k \log k)} n$ and
there exists $(j,g) \in \randfamily$ such that $j = \jmaj(f^{\beta,\ast})$ and $g$ agrees with $f^{\beta,\ast}$ on
$A^\ast \cup B^\ast$. Furthermore, for every element $(j,g) \in \randfamily$, $g$ agrees with $f^\adh$
on $\adh(t)$.
\end{claim}
\begin{proof}
First, we iterate over all choices of nonnegative integers $j \in [p]$ and $a_1,a_2, \ldots, a_{p}$
such that $\sum_{i=1}^{p} a_i \leq 3k+k(k+p)$ and $\sum_{i \in [p] \setminus \{j\}} a_i \leq 3k$. 
Clearly, there are $2^{\Oh(k)}$ options.
For a fixed choice of $j$ and $(a_i)_{i=1}^{p}$ we invoke Lemma~\ref{lem:random2}
for $U = \beta(t) \setminus \adh(t)$ and integers $r = p$, $(a_i)_{i=1}^{p}$, obtaining a family
$\randfamily'$. For every $g' \in \randfamily'$, we insert $(j, g' \cup f^\adh)$
  into $\randfamily$.

The bound on the size of the output family $\randfamily$ follows from bound of Lemma~\ref{lem:random2}
and the inequality $log^k n \leq 2^{\Oh(k \log k)} n$. 
Finally, note that the promised pair $(j,g)$ will be generated for the choice of
$j = \jmaj(f^{\beta,\ast})$ and $a_i = |(f^{\beta,\ast})^{-1}(i) \cap (A^\ast \cup B^\ast)|$ for every $i \in [p]$.
\cqed\end{proof}

Invoke the algorithm of Claim~\ref{cl:sc:random}, obtaining a family $\randfamily$. We say
that $(j,g) \in \randfamily$ is \emph{lucky} if $f^{\beta,\ast}$ exists, $j = \jmaj(f^{\beta,\ast})$, and $f^{\beta,\ast}$
agrees with $g$ on $A^\ast \cup B^\ast$. 

Consider now an auxiliary graph $H$ with $V(H) = \beta(t)$ and $uv \in E(H)$ if and only if
$u \neq v$ and there exists a constraint $\Gamma \in \cnstr$ with $u,v\in X_\Gamma$.
By the definition of constraints $\Gamma(e)$, we have that $G_t[\beta(t)]$ is a subgraph of
$H$, but in $H$ we also turn all adhesions $\adh(s)$ for $s \in Z$ into cliques.

For a pair $(j,g) \in \randfamily$, we define $\Sigma(j,g) := g^{-1}([p] \setminus \{j\})$.
Observe the following.

\begin{claim}\label{cl:sc:stains}
For a lucky pair $(j,g)$,
every connected component of $H[\Sigma(j,g)]$ is either completely contained
in $(f^{\beta,\ast})^{-1}(j)$ or completely contained in $A^\ast$.
\end{claim}
\begin{proof}
Assume the contrary, and let $uv \in E(H)$ be an edge violating the condition. By symmetry, assume $f^{\beta,\ast}(u) \neq j$.
Then, since $(j,g)$ is lucky, we have that $u \in A^\ast$. Hence $v \notin A^\ast$, that is, $f^{\beta,\ast}(v) = j$. 
By the definition of $H$, there exists a constraint $\Gamma \in \cnstr$ with $u,v \in X_{\Gamma}$ (either $\Gamma = \Gamma(uv)$ or
$\Gamma = \Gamma(s)$ for some $s \in Z$ with $u,v \in \adh(s)$). Consequently, $\Gamma$ is touched, and $v \in B^\ast$.
However, then from the fact that $(j,g)$ is lucky it follows that $g(v) = j$, a contradiction.
\cqed\end{proof}


\end{proof}


==> decomposition-edge.tex <==
\begin{proof}[Proof of Lemma~\ref{lem:edge-cut}.]
If the vertices of $S$ are present in more than one connected component of $G$, then we can return an edge cut of order zero with some vertices of $S$ on both sides of the cut, and we are done.
Otherwise, as the statement is trivial for $S = \emptyset$, we can assume $G$ is connected by focusing on the single connected component of $G$ that contains all vertices of $S$.
Furthermore, since the problem is easily solvable in time $n^{\Oh(k)}$, we assume $k \geq 2$.

We start with a regularization step.

\begin{claim}\label{cl:ABreg}
If there exists an edge cut $(A,B)$ as in the lemma statement, then there exists one where
$G[A]$ and $G[B]$ are connected.
\end{claim}
\begin{proof}
By definition, every edge of $E(A,B)$ has one endpoint in $A$ and one endpoint in $B$.
Since $|B \cap S| > |E(A,B)|$, there exists a connected component $C_B$ of $G[B]$ such that $|C_B \cap S| > |E(V(G) \setminus C_B,C_B)|$. Also, note that
$E(V(G) \setminus C_B,C_B) \subseteq E(A,B)$ as $C_B$ is a connected component of $G[B]$ and clearly $A \cap S \subseteq (V(G) \setminus C_B) \cap S$.
Thus, the cut $E(V(G) \setminus C_B,C_B)$ also satisfies the requirements of the lemma. Consequently, we can assume that $G[B]$ is connected.

We now perform exactly the same operation, but with the roles of $A$ and $B$ swapped, using a component $C_A$ of $G[A]$.
By the connectivity of $G$, since $G[B]$ is connected, $G-C_A$ is connected as well. Consequently, after performing the same operation using the component $C_A$,
both $G[A]$ and $G[B]$ are connected.
\cqed\end{proof}

We note here that the main reason why we are not able to get an exact FPT algorithm for checking $(k,k)$-unbreakability (as opposed to $(k,k)$-edge unbreakability), 
is that the analogue of Claim~\ref{cl:ABreg} fails for vertex cuts.

For a connected component $D$ of $G-S$, by $G_D$ we denote the graph $G[N_G[D]] \setminus E(G[N_G(D)])$, that is, the subgraph of $G$ induced by all edges with at least one endpoint in $D$.
Note that graphs $G_D$ for different components $D$ are pairwise edge-disjoint.

Assume that an edge cut satisfying the conditions of the lemma exists,
       and fix one such edge cut $(A,B)$. By Claim~\ref{cl:ABreg},
we can additionally assume that both $G[A]$ and $G[B]$ are connected.
Let $\ell = |E(A,B)|$.

We say that a component $D$ of $G-S$ is \emph{touched} if at least one edge of $G_D$ is present in $E(A,B)$,
    and a vertex $t \in S$ is \emph{touched} if either $t$ is an endpoint of an edge of $E(A,B)$,
or there exists a touched component $D$ with $t \in N(D)$.
Note that every component $D$ gives raise to at most $k$ touched vertices, while every edge of $E(A,B) \cap E(G[S])$ gives raise to two touched vertices. Since $|E(A,B)| \leq k$,
there are at most $k$ touched components of $G-S$ and at most $k^2$ touched vertices of $S$.

We construct an auxiliary graph $H$ as follows. We take $V(H) = S$ and two vertices $u,v \in S$
are connected by an edge in $H$ if $uv \in E(G)$ or there exists a component $D$
of $G-S$ such that $u,v\in N_G(D)$. The graph $H$ is sometimes called the \emph{torso} of $S$ in 
literature.

Since $G[A]$ and $G[B]$ are connected, $H[A \cap S]$ and $H[B \cap S]$ are connected as well.
Let $S_A$ (resp. $S_B$) be an arbitrary set of $\ell+1$ vertices of $A \cap S$ (resp. $B \cap S$)
such that $H[S_A]$ (resp. $H[S_B]$) is connected.
Finally, let $C$ be the set of all touched vertices of $S$ that are not contained in $S_A \cup S_B$.

We apply Lemma~\ref{lem:random2} to the universe $S$ with $r=3$, $a_1=a_2=k+1$
and $a_3=c=k^2$. In time $2^{\Oh(k \log k)} n \log^2 n$ we obtain a family $\randfamily$
of $2^{\Oh(k \log k)} \log^2 n$ functions $f \colon S \to \{1,2,3\}$ such that 
there exists $f \in \randfamily$ with
$S_A \subseteq f^{-1}(1)$, $S_B \subseteq f^{-1}(2)$
and $C \subseteq f^{-1}(3)$.
Note that if this is the case, then $S_A$ is contained in one connected component of
$H[f^{-1}(1)]$ and $S_B$ is contained in one connected component of $H[f^{-1}(2)]$.

We observe the following.
\begin{claim}\label{cl:edge:use-f}
If $f \colon S \to \{1,2,3\}$ is such that 
$S_A \subseteq f^{-1}(1)$, $S_B \subseteq f^{-1}(2)$,
and $C \subseteq f^{-1}(3)$, then
the connected component of $H[f^{-1}(1)]$ containing $S_A$ is completely contained in $A \cap S$
and, symmetrically, 
the connected component of $H[f^{-1}(2)]$ containing $S_B$ is completely contained in $B \cap S$.
\end{claim}
\begin{proof}
The claim follows from an observation that for every edge $v_Av_B \in E(H)$ with $
v_A \in A$ and $v_B \in B$ we have that $v_A$ and $v_B$ are touched and, consequently,
$v_A \in S_A \cup C$ and $v_B \in S_B \cup C$. Hence, the connected component of $H[f^{-1}(1)]$
containing $S_A$ cannot contain any vertex of $B$, and a symmetrical claim holds for $H[f^{-1}(2)]$.
\cqed\end{proof}

By iterating over all the less than $|\randfamily| \cdot |S|^2 = 2^{\Oh(k \log k)} n^2 \log^2 n$
options, we guess the function $f \in \randfamily$ satisfying the assumptions of Claim~\ref{cl:edge:use-f} and the connected components $A_0$ and $B_0$ of $H[f^{-1}(1)]$ and $H[f^{-1}(2)]$, respectively,
that contain $S_A$ and $S_B$, respectively.
Note that $|A_0| \geq |S_A| = \ell+1$ and $|B_0| \geq |S_B| = \ell+1$. On the other hand,
since $A_0 \subseteq A$ and $B_0 \subseteq B$, while $|E(A,B)| \leq \ell$, one can in polynomial
time find an edge cut $(A',B')$ of order at most $\ell$ with $A_0 \subseteq A'$ and $B_0 \subseteq B'$. While we may not necessarily obtain $(A',B') = (A,B)$, the cut $(A',B')$ satisfies the desired properties
and can be returned by the algorithm.
This finishes the proof of Lemma~\ref{lem:edge-cut}.
\end{proof}




==> decomposition-vertex.tex <==
\begin{proof}[Proof of Lemma~\ref{lem:separations}.]
Similarly as in the proof of Lemma~\ref{lem:edge-cut}, we can restrict our attention
to connected graphs $G$.
That is, if the vertices of $S$ are present in more than one connected component,
then we can return a separation of order zero with some vertices of $S$ on both sides of the cut, and we are done.
Otherwise, as the statement is trivial for $S = \emptyset$, we can assume $G$ is connected by focusing on the single connected component of $G$ that contains all vertices of $S$.

As in the proof of Lemma~\ref{lem:edge-cut}, 
   we define $H$ to be the torso of $S$ in $G$. 
That is, we take $V(H) = S$ and two vertices $u,v \in S$
are connected by an edge in $H$ if $uv \in E(G)$ or there exists a component $D$
of $G-S$ such that $u,v\in N_G(D)$.

Assume that there exists a separation $(A,B)$ of order at most $k$ and such that  $|A \cap S|, |B \cap S| > 2^k k$; fix one such separation.
We say that a component $D$ of $G-S$ is \emph{touched} if $D \cap A \cap B \neq \emptyset$.
A vertex $t \in S$ is \emph{touched} if either $t \in A \cap B$ 
or there exists a touched component $D$ with $t \in N(D)$.
Note that every component $D$ gives raise to at most $k$ touched vertices.
There are at most $k$ touched components of $G-S$ and at most $k^2$ touched vertices of $S$.

We now consider two cases. 

\paragraph*{Case 1:} We first assume that both $H[(A \setminus B) \cap S]$ and
$H[(B \setminus A) \cap S]$
contain connected components of size at least $k+1$ each.
Let $S_A \subseteq (A \setminus B) \cap S$ be a set of $k+1$ vertices such that $H[S_A]$ is connected,
and similarly define $S_B \subseteq (B \setminus A) \cap S$.
Let $C$ be the set of touched vertices that are not contained in $S_A \cup S_B$.

We apply Lemma~\ref{lem:random2} to the universe $S$ with $r=3$, $a_1=a_2=k+1$
and $a_3=c=k^2$. In time $2^{\Oh(k \log k)} n \log^2 n$ we obtain a family $\randfamily$
of $2^{\Oh(k \log k)} \log^2 n$ functions $f \colon S \to \{1,2,3\}$ such that 
there exists $f \in \randfamily$ with
$S_A \subseteq f^{-1}(1)$, $S_B \subseteq f^{-1}(2)$
and $C \subseteq f^{-1}(3)$.
Note that if this is the case, then $S_A$ is contained in one connected component of
$H[f^{-1}(1)]$ and $S_B$ is contained in one connected component of $H[f^{-1}(2)]$.

The following claim is straightforward by the definition of touched vertices.
\begin{claim}\label{cl:vertex:use-f}
If $f \colon S \to \{1,2,3\}$ is such that 
$S_A \subseteq f^{-1}(1)$, $S_B \subseteq f^{-1}(2)$,
and $C \subseteq f^{-1}(3)$, then
the connected component of $H[f^{-1}(1)]$ containing $S_A$ is completely contained in $(A \setminus B) \cap S$
and, symmetrically, 
the connected component of $H[f^{-1}(2)]$ containing $S_B$ is completely contained in $(B \setminus A) \cap S$.
\end{claim}

By iterating over all the less than $|\randfamily| \cdot |S|^2 = 2^{\Oh(k \log k)} n^2 \log^2 n$
options, we guess the function $f \in \randfamily$ satisfying the assumptions of Claim~\ref{cl:vertex:use-f} and the connected components $A_0$ and $B_0$ of $H[f^{-1}(1)]$ and $H[f^{-1}(2)]$, respectively, that contain $S_A$ and $S_B$, respectively.
Note that $|A_0| \geq |S_A| = k+1$ and $|B_0| \geq |S_B| = k+1$. On the other hand,
since $A_0 \subseteq (A \setminus B)$ and $B_0 \subseteq (B \setminus A)$, while $|A \cap B| \leq \ell$, one can in polynomial
time find an separation $(A',B')$ of order at most $\ell$ with $A_0 \subseteq A'$ and $B_0 \subseteq B'$. While we may not necessarily obtain $(A',B') = (A,B)$, the separation
$(A',B')$ satisfies the desired properties
and can be returned by the algorithm.
This finishes the description of the first case.
Let us note here that in this case we did not use the assumption $|A \cap S|, |B \cap S| > 2^k k$.

\paragraph*{Case 2:} We now assume that either every every connected component of $H[(A \setminus B) \cap S]$
has at most $k$ vertices, or this holds for $H[(B \setminus A) \cap S]$.
By symmetry, without loss of generality assume the former.
In particular, this implies that every connected component of $G[A \setminus B]$ has
at most $k$ vertices of $S$.

We now observe the following.
\begin{claim}\label{cl:vertex:2k}
If there exists a separation $(A,B)$ of order at most $k$ with $|A \cap S|, |B \cap S| > 2^k k$ such that every connected component of $G[A \setminus B]$ has at most $k$ vertices from $S$,
then there exists a separation $(A',B')$
of order at most $k$ such that $A' \subseteq A$, $B' \supseteq B$ and thus $|B' \cap S| > 2^k k$, $|(A' \setminus B') \cap S| > k$, and every connected component $A_0$ of $G[A' \setminus B']$ satisfies $|A_0 \cap S| \leq k$ and $N_G(A_0) = A' \cap B'$.
\end{claim}
\begin{proof}
Let $\mathcal{A}$ be the family of connected components of $G[A \setminus B]$, and for every nonempty
$X \subseteq A \cap B$ let $\mathcal{A}_X$ be the family of those components $A_0 \in \mathcal{A}$ for which $N_G(A_0) = X$.
By the Pigeonhole Principle, if $|A \cap S| > 2^k k$, so in particular $|(A \setminus B) \cap S| > (2^k-1)k$, then there exists $X$ for which $\bigcup \mathcal{A}_X$ contains more than $k$ vertices of $S$.
Thus, we can set $A' = X \cup \bigcup \mathcal{A}_X$ and $B' = V(G) \setminus \bigcup \mathcal{A}_X$.
\cqed\end{proof}
Thus, we can focus on finding a separation $(A',B')$ as in Claim~\ref{cl:vertex:2k}. 
The following observation simplifies future work.
\begin{claim}\label{cl:vertex:X-in-S}
Let $(A,B)$ be a separation of order at most $k$ with $|A \cap S|, |B \cap S| > 2^k k$ such that every connected component of $H[(A \setminus B) \cap S]$ has at most $k$ vertices from $S$.
Let $(A',B')$ be a separation given by Claim~\ref{cl:vertex:2k} for the separation $(A,B)$.
Then $A' \cap B' \subseteq S$.
\end{claim}
\begin{proof}
Assume the contrary: there exists a connected component $D$ of $G-S$ with a vertex
$v \in D \cap A' \cap B'$. Let $A_0$ be an arbitrary connected component of $G[A' \setminus B']$
with $A_0 \cap S \neq \emptyset$; such a connected component
$A_0$ exists as $|(A' \setminus B') \cap S| > k$.
Since $N_G(A_0) = A' \cap B'$, there exists a vertex $u \in S \cap A_0 \cap N_G(D)$.
However, since $N_G(D)$ is a clique in $H$, all such vertices $u$ for different choice of $A_0$ lie in the same connected component of $H[(A' \setminus B') \cap S]$.
Obviously, $H[A_0 \cap S]$ is connected as $G[A_0]$ is connected.

We infer that all vertices of $(A' \setminus B') \cap S$ lie in a single connected component of
$H[(A' \setminus B') \cap S]$. Since $A' \subseteq A$ and $B' \supseteq B$, while $|(A' \setminus B') \cap S| > k$, we infer that
there exists a connected component of $H[(A \setminus B) \cap S]$ that contains more than $k$ vertices. This is the desired contradiction.
\cqed\end{proof}

Let $A_0$ an arbitrary connected component of $G[A' \setminus B']$ containing vertices of $S$.
Claim~\ref{cl:vertex:X-in-S} together with $N_G(A_0) = A' \cap B'$ implies that
\begin{equation}\label{eq:vertex:final}
A' \cap B' = N_H(A_0 \cap S).
\end{equation}
Let $C$ be the set of touched vertices of $S$ that are not contained in $A_0$. 
We invoke Lemma~\ref{lem:random} for the universe $S$ and parameters $a=k+1$ and $b=k^2$, obtaining a family $\randfamily$ of subsets of $S$
such that there exists $S \in \randfamily$ with $A_0 \cap S \subseteq S$ and $S \cap C = \emptyset$.
A direct consequence of the definition of $C$ and~\eqref{eq:vertex:final} is that for such $S \in \randfamily$, the set $A_0 \cap S$ is a connected 
component of $H[S]$. Thus, by iterating over all sets $S \in \randfamily$ and connected components of $H[S]$, we can guess the set $A_0 \cap S$,
          by~\eqref{eq:vertex:final}, obtain $A' \cap B' = N_H(A_0 \cap S)$.
Finally, given $A' \cap B'$, it is straightforward to find a candidate for $A'$ by collecting a minimal set of components $\hat{A}$ of $G-(A' \cap B')$ with $N(\hat{A}) = A' \cap B'$
and $|\hat{A} \cap S| \leq k$ such that the union of these components contains more than $k$ vertices of $S$.
Note that in this process we might incidentally use some vertices of $B' \cap S$, however we will use at most $2k$ of them,
hence the remainder of the graph will contain enough vertices of $S$ for the lemma to hold.
This finishes the proof of the second case, and the whole lemma.
\end{proof}


